Elementary Particles and Plasma in the First Hour of the Early Universe

This dissertation aims to deepen the understanding of the primordial composition of the Universe in the temperature range 300 MeV>T>0.02 MeV. I exploit known properties of elementary particles and apply methods of kinetic theory and statistical physics to advance the understanding of the cosmic plasma. Within the Big Bang model, we begin by considering the Universe being a highly energetic fireball, an ultra-relativistic plasma exhibiting distinct properties. Fundamental particles such as quarks, leptons, and even heavier gauge bosons play a crucial role in the understanding of the early Universe. Our research focuses on the investigation of these fundamental particles as constituents of the dense Universe plasma during the epoch which transits from primordial quark-gluon plasma to the era of normal hadron matter, passing through the decoupling of neutrinos and addressing in detail the electron-positron antimatter plasma.

==> abstract.tex <==
%This is where the body of your abstract goes, limited to 150 words
%for a thesis, and 350 words for a dissertation or document.  The
%word count limits apply to the regular Abstract in the thesis and
%to the separate Special Abstract.  Use the same text for both; just
%adjust the margins and heading.  The abstract should summarize your
%work.  The UMI booklet listed in the resources section of the U of
%A manual provides some writing tips.  The abstract for a dissertation
%or document may be longer than one page; word count is more important
%than page length in this section.

%If you are doing a paper submission, submit one copy of the special 
%abstract, and two extra copies of your title page, in the box with 
%the final copies of your thesis.  If you are doing an electronic
%submission, you can ignore the special abstract.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In this dissertation, we study the evolution and properties of the early universe from temperature $0.3\,\mathrm{GeV}>T>20\,\mathrm{keV}$.  Specifically, we aim to explore the connection between fundamental particles and cosmic plasma in the early universe. According to the standard model of the "Big Bang," the universe began as a highly energetic fireball with an immensely high temperature and energy density. Consequently, an ultra-relativistic plasma was generated, exhibiting distinct properties as the universe expanded and cooled.  When the universe is hot and dense, fundamental particles (such as quarks, leptons, and gauge bosons) play a crucial role in understanding the early universe. These elementary particles were abundantly present shortly after the Big Bang and their interactions governed the dynamics of the early universe. Our research focus on investigation of these fundamental particles within the context of cosmic plasma and offering valuable insights into the evolution of the early universe.


This work aims to deepen the understanding of the primordial composition of the Universe in the temperature range $300\,\mathrm{MeV}>T>0.02\,\mathrm{MeV}$. In the following I exploit known properties of elementary particles and apply methods of kinetic theory and statistical physics to advance the understanding of  the  cosmic plasma. Within the Big Bang model the Universe began as a highly energetic fireball with an immensely high temperature and energy density. Consequently, an ultra-relativistic plasma was generated, exhibiting distinct properties as the Universe expanded and cooled.  When the Universe is hot and dense, fundamental particles (such as quarks, leptons, and gauge bosons) play a crucial role in understanding the early Universe. These elementary particles were abundantly present once the temperature dropped below $T=130$\,GeV. Their interactions governed the dynamics of the early Universe. Our research focuses on investigation of these fundamental particles during the epoch which transits from primordial quark-gluon degrees of freedom to the era of normal matter plasma (H$^+$, He$^{+}$, $e^-$). Our findings will offer valuable insights into the properties of the early Universe governing the properties of matter surrounding us today.

In chapter \ref{Introduction} the properties of the Universe during the `first hour' are described. I do not discuss diverse ideas about the origin of the Universe or how it emerged in thermal state.  I begin with  primordial Quark Gluon Plasma (QGP), continue to address the evolution of formed hadrons, of leptons, and the  decoupling of neutrinos. I consider as well the stage where the electron-positron plasma is dominant. Most of these results depend on ambient (photon) temperature only. The standard cosmological  Friedmann-Lemaitre-Robertson-Walker (FLRW)  model of the Universe is also introduced allowing the connection of the magnitude of temperature $T$ to the age of the Universe $t$ and the understanding of the speed of temperature change. 

I address in particular bottom and charm quarks near to the QGP transformation to hadrons (hadronization temperature $T_H=150$\,MeV) in chapter \ref{Bottom}. I examine the relaxation time for the production and decay of bottom/charm quarks as a function of temperature from $300\,\mathrm{MeV}>T>150\,\mathrm {MeV}$. Of particular interest to me is that the bottom quarks are not in their chemical equilibrium.%, which provide
%a strong motivation to explore the physics of baryon nonconservation involving the
%bottomnium mesons or/and bottom quarks in early universe.
%I use this to suggest that the baryon asymmetry may relate to the bottom quark non-equilibrium abundance in the early Universe. 

In chapter \ref{Strangeness}, I examine the strange particle composition of the expanding early Universe in the hadron epoch $150\,\mathrm{MeV}\ge T\ge 10$\,MeV, then investigate the freeze-out temperature for strangeness-producing  by comparing the relevant reaction rates to the Hubble expansion rate and show that strangeness are kept in equilibrium via weak, electromagnetic, and strong interactions in the early Universe until $T\approx13$ MeV.

In chapter \ref{Neutrino}, the matrix elements for neutrino coherent/incoherent scattering with matter and their application in early Universe are studied in detail. An overview of neutrino freeze-out process in early Universe is presented. After neutrino freeze-out, I examine the relation between the effective number of neutrinos $N^{\mathrm{eff}}_\nu$ and lepton asymmetry $L$ in the Universe and its impact on Universe expansion. %To be specifically, I explore relation between the large cosmological lepton asymmetry and the effective number of neutrinos $N^{\mathrm{eff}}_\nu$ in early Universe.


In chapter \ref{Electron}, I examine the dynamical picture of charged leptons $\mu^\pm$ and $e^\pm$ in the early Universe and show that the persistence temperature for $\mu^\pm$ in the early Universe is $T = 4.2 $ MeV, and the $e^+$ abundance can persist in the early Universe at relatively low value  $T\approx20\,\mathrm{keV}$. Given the dense electron-positron plasma in the early Universe, I study the damping rate and investigate the magnetization process within dense electron-positron plasma in the early Universe.

In chapter~{\ref{Outlook}}, I address the ongoing and prospective research projects intended for future publication including: The application of nonequilibrium bottom quark; Population of Higgs in the early Universe; Extra neutrino from microscopic processes after freeze-out; Self-consistent relaxation rate for electron-positron plasma. Finally, we summarize our important results and outlook for future study in chapter \ref{Summary}.


==> acknowledgements.tex <==
%add acknowledgements here

%Thanks to advisor
%Thanks to our group
%Thanks to Commitiee
%Thanks to my frirends

I would like to thank my adviser and mentor, Professor Johann Rafelski for his patience, encouragement, and dedication in helping me achieve this goal. This dissertation could not have happened without his great insight into so many areas of physics and kindly support. He stands as a remarkable role model in the science and life. His passion and tireless dedication to the field of physics, unwavering optimism, and professional working attitude have left an enduring mark on my approach to research and life attitude. I am grateful for all these invaluable lessons I have learned from him during my journey with him in Arizona. My gratitude also goes to his wife, Victoria Grossack, for hosting many memorable group meetings at their house throughout the years.



I would like to extend my thanks to the research colleagues and close collaborators in Prof. Rafelski’s group: (in alphabetical order) Stefan Evans,  Martin Formanek, Shelbi J Foster, Chris Grayson, Will Price, Andrew Steinmentz for many physics discussions and their friendship. I would like to thank Dr.Jeremiah Birrell for the physics discussions and help when I was in Taiwan and Arizona. I would like to express my gratitude to Rohit Singh for his generous assistance and support during my time as a Teaching Assistant. 


I would like to thank my fiends from Taiwan and Tucson for their friendship and company for my life and PhD journey in Tucson (in alphabetical order): Maxwell Cui, Miwa Clucas, Lia Chen, Angelica Escoto, Jingwei Liu, Yang Liu, Yen-Wei Liu, Carl Dean Orfield, Chung-Yi Tasi, Wei-Leong Tee, Bianca Wang. 
Furthermore, I would like to express my gratitude to my sister and her family, Irene Yang, Jay Lee, and Summer Lee for their generous support and help. 



Finally, I would like to express my thanks to my thesis committee for kindly accepting to take part, for reading this dissertation, and for providing me with helpful advice for improving its contents. 



%Finally, thank you, the reader, for joining me on these pages in what has been a substantial and exciting part of my life.








==> dedication.tex <==
\begin{center}
\emph{I dedicate this work to my parents for their invaluable support and encouragement, which sustained me through the highs and lows of my journey.}
%One page maximum.
\end{center}


